Is Stellar As Secure As You Think?

Stellar is one of the top ten cryptocurrencies in terms of market capitalization. It adopts a variant of Byzantine fault tolerance (BFT), named federated Byzantine agreement (FBA), which generalizes the traditional BFT algorithm to make it more suitable for open-membership blockchains. To this end, FBA introduces a quorum slice concept, which consists of a set of nodes. In FBA, a node can complete one consensus round when it receives specific messages from nodes in a quorum slice appointed by the node. In this study, we analyze FBA, whose security is highly dependent on the structure of quorum slices, and demonstrate that it is not superior to the traditional BFT algorithm in terms of safety and liveness. Then, to analyze the security of the Stellar consensus protocol (SCP), which is a construction for FBA, we investigate the current quorum slices in Stellar. We analyze the structure of quorum slices and measure the influence of each node quantitatively using two metrics, PageRank (PR) and the newly proposed NodeRank (NR). The results show that the Stellar system is significantly centralized. Thereafter, to determine how the centralized structure can have a negative impact on the Stellar system, we study the cascading failure caused by deleting only a few nodes (i.e., validators) in Stellar. We show that all of the nodes in Stellar cannot run SCP if only two nodes fail. To make matters worse, these two nodes are run and controlled by a single organization, the Stellar foundation.

==> buffer/methodology.tex <==
\section{Methodology}
\label{sec:methodology}

In this section, we describe what data we collected and how we collected it.
To collect data, we participated in main network of Stellar as a validator who directly participates in voting.
To be a validator, we had to generate own seed value through Stellar API and then registered it to our configuration file.
We then had to make own quorum set consisting of nodes that we trust and add the quorum set in the configuration file.
Then we could start running the validator node and collecting whole information about the Stellar network.
Through this, we could collect data about peers' IP addresses, quorum sets in Stellar, process of voting.

\smallskip
\noindent\textbf{Data about quorum sets in Stellar: } 
Fig.~\ref{fig:quorum_set_log} is the data about existing quorum sets in main network of Stellar.
Each quorum has its own hash value, "t", and "v". 
The first 6 characters of hash value are used as the ID of the corresponding quorum set.
In addition, "t" represents the concept of threshold and "v" represents members of the quorum sets.
As an example, a1e4f6 is the ID of the first quorum set in Fig.~\ref{fig:quorum_set_log}. 
Because the value of "t" is 4, if more than 4 members out of those 5 members vote on the statement $a$, the creator of "a1e4f6" quorum set would agree with the statement $a$ ultimately.
The members of this quorum set are \textit{GCXLL, eno, sdf\_watcher1, sdf\_watcher2,} and \textit{sdf\_watcher3}. 
Moreover, we were able to identify nested quorum set which is quorum set in a quorum set. 
Each nested quorum set also has to have each own threshold value.

\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{figure/quorum_set_figure.png}
\caption{Data about quorum sets in main network.}
\label{fig:quorum_set_log}
\end{figure}

\smallskip
\noindent\textbf{Data about consensus phases in Stellar: } 
Fig.~\ref{fig:voting_phrases} shows current ongoing phase of consensus such as $nominate$, $prepare$, $confirm$ or $externalize$ for each node about each sequence of slot. 
Through this log, we could know not only the phase of consensus but also who has made what quorum set. 
In Fig.~\ref{fig:voting_phrases}, the name after "ENV@" is the node who made its quorum set which hash value is number after "D: ".
For example, in the very first paragraph from Fig.~\ref{fig:voting_phrases}, \textit{tempo.eu.com} made quorum set which hash value is 8ba0fb. 
We could check members in quorum set 8ba0fb from data log in Fig.~\ref{fig:quorum_set_log}.

\smallskip
\noindent\textbf{Data from Stellar database: }
In the database of Stellar, we could gather lots of other data that we couldn't collect from the log file.
There are IPs of peers who are running node of Stellar, hash value of transactions in blockchain, and information about the history.


\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{figure/voting_phase.png}
\caption{Data about phases of federated voting.}
\label{fig:voting_phrases}
\end{figure}



==> future.tex <==
\section{Future Works}
\label{sec:future}

In this paper, we showed that quorum structure in Stellar is totally centralized.
Therefore, we could fail the Stellar network completely by deleting some of those centralized nodes.
Even though we only focused on quorum structure in this paper, there can be other attacks such as double spending attack on different fields.
The double spending attack is one of the most troublesome attacks in cryptocurrency, and it can happen on Stellar in some cases.
Therefore, we are going to find some scenarios that this attack can happen. 
Furthermore, we are going to find additional conditions that have to be satisfied when making quorums to prevent both cascading attack and double spending attack.\\
It is important to find the optimal value of the threshold for the security on Stellar.
However, it is still an open problem because there is a trade-off between liveness and safety. 
Therefore, it can be challenging to satisfy safety and liveness at the same time with the threshold.
If the value of the threshold is high for the safety, the cascading attack can happen.
On the other hand, if the value of the threshold is low for the sake of liveness, the double spending attack can happen.
Accordingly, finding the optimal value of the threshold can be our remaining work to do.

==> result.tex <==
\section{Result Analysis}
\label{sec:result}

In this section, we analyze and summarize results of data analysis and cascading failure.

\subsection{Value of $x$-crushed}

In section ~\ref{sec:theoretical}, we define $x$-crushed system.
Considering the fact that if two out of 62 validators in the Stellar network fails, then the entire system will be collapsed, we can say the value of $x$-crushed in Stellar system is 3-crushed (i.e. 2/62*100 = 3.2).
To compare Stellar with other blockchain protocols, we summarize x-crushed values of top 10 cryptocurrencies at the time of writing.

\begin{table}[t]
\centering
\caption{Value of $x$-crushed in Top 10 Cryptocurrencies.}
\begin{tabular}{|c|c|c|c|}
\hline
Rank          &Protocol      &$x$-crushed (\%)      & Number of Ill-behaved Nodes   \\
\hline \hline
1              &Bitcoin      &0                   &2   \\
3              &Ethereum     &0                   &2    \\
4              &EOS          &33                  &7     \\
5              &Bitcoin Cash &0                   &2     \\
6              &Litecoin     &0                   &3      \\
7              &Tether       &0                   &2      \\
8              &TRON         &33                  &9     \\
9              &Stellar      &3                   &2      \\
10             &Bitcoin SV   &0                   &2       \\
\hline
\end{tabular}
\label{table:purposeOfValidator}
\end{table}

In summary, we see what number of validators have to be ill-behaved to make entire system cannot make a consensus, and find out the value of $x$ is significantly small.


\subsection{Centralized quorum slice structure}
As we said before, when all the well-behaved nodes are in group \textit{C}, the system can be secure under the current Stellar protocol.
From the perspective of Stellar protocol, this can be determined by quorum slices structure (or slice network).
As the quorum slice network is more decentralized, less well-behaved nodes will be affected by ill-behaved nodes leading for almost all the well-behaved nodes to stay in group \textit{A}.

Usually, if there are significantly small number of nodes in each quorum slice or in the network, or if the power is biased to a few validators (i.e., in Stellar, the power means how much the validator is trusted by others), the quorum slice network is considered as centralized.
Therefore, we can say that current Stellar is highly centralized quorum slice structure, because the number of nodes in slices is small and power distribution is biased. 
Furthermore, we check that with the current quorum slice network, the Stellar is 3-crushed system, which means failing two ill-behaved nodes can lead for all the remaining well-behaved nodes to be in group \textit{B}.


To make slice structure decentralized, the number of nodes in slices should be small and each validator should have even power distribution.
In case of Stellar, because it does not satisfy both, the degree of centralization in Stellar is high.
%On the other hand, in case of delegated proof of stake (DPoS), such as EOS, even though there are only 21 valdiators (block producers) in one round but the 21 nodes have even power distribution.
%Furthermore, in case of proof of work (PoW), such as Bitcoin, even though the power distribution is highly biased (e.g. only two mining pools account for more than 33\% of the total power), there are large number of miners~\ref{number_of_miners}.
%Therefore, EOS or Bitcoin satisfies at least one condition, we can say that those are more decentralized than Stellar.
If the Stellar has more validators and all of them are included in slices with similar number of times, it can be more decentralized than the current status quo.
However, it is not easy to make Stellar satisfy those two conditions with the current Stellar protocol.
Firstly, because there is no incentivization, nodes that would not receive any external profit tend not to participate in the Stellar network.
Secondly, with the trust model, it is hard for all validators to be trusted with similar number of times because user tends to select validator that is popular or related with itself.
More specifically, most of the current nodes participating in Stellar are nodes that collaborate with Stellar or provide services using Stellar.
Thus, they are tend to trust nodes that are run by Stellar foundation.
If you see the current status quo, we can see that at least one of \textit{sdf\_validator} nodes is included in all slices.
This state shows that if the reasons why nodes work as validators are similar, then they tend to choose similar validators which makes Stellar network more centralized.
Hence, unless there is no incentivization system that makes many normal people actively participate in the network as a validator, it will be hard for the quorum slice network to be decentralized.
In addition, even if there is an incentivization (so that there are many non-profit validators), it can not be sure that users will include various validators that exist equally in the slice.


%In fact, there are some other suggestions to make quorum slice network decentralized.
%Changing quorum slices systematically so that every validators have similar power can be possible, but than 
%Sybil attack can happen because some validators that are not trusted by others must be included too.
%Therefore, it is dilemma.


